Faster Differentially Private Samplers via R\'enyi Divergence Analysis of Discretized Langevin MCMC

Various differentially private algorithms instantiate the exponential mechanism, and require sampling from the distribution $\exp(-f)$ for a suitable function $f$. When the domain of the distribution is high-dimensional, this sampling can be computationally challenging. Using heuristic sampling schemes such as Gibbs sampling does not necessarily lead to provable privacy. When $f$ is convex, techniques from log-concave sampling lead to polynomial-time algorithms, albeit with large polynomials. Langevin dynamics-based algorithms offer much faster alternatives under some distance measures such as statistical distance. In this work, we establish rapid convergence for these algorithms under distance measures more suitable for differential privacy. For smooth, strongly-convex $f$, we give the first results proving convergence in R\'enyi divergence. This gives us fast differentially private algorithms for such $f$. Our techniques and simple and generic and apply also to underdamped Langevin dynamics.

==> intro-new.tex <==

\section{Introduction}

%Various differentially private algorithms instantiate the exponential mechanism, and require sampling from the distribution $\exp(-f)$ for a suitable function $f$. When the domain of the distribution is high-dimensional, this sampling can be challenging. Using heuristic sampling schemes such as Gibbs sampling does not necessarily lead to provable privacy. When $f$ is convex, techniques from log-concave sampling lead to polynomial-time algorithms, albeit with large polynomials. Langevin dynamics-based algorithms offer much faster alternatives under some distance measures such as statistical distance. In this work, we establish rapid convergence for these algorithms under distance measures more suitable for differential privacy. For smooth, strongly-convex $f$, we give the first results proving convergence in R\'enyi divergence and show stronger results under $(\eps, \delta)$-DP. This gives us fast differentially private algorithms for such $f$. Our techniques and simple and generic and apply also to underdamped Langevin dynamics.

The Exponential Mechanism~\citep{McSherryT07} is a commonly-used mechanism in differential privacy~\citep{DworkRbook}. There is a large class of mechanisms in the differential privacy literature that instantiate the Exponential Mechanism with appropriate score functions, use it as a subroutine, or sample from $\exp(-f)$ for some function $f$. This family includes differentially private mechanisms for several important problems, such as PCA~\citep{ChaudhuriSS, KapralovT}, functional PCA~\citep{AwanKRS}, answering counting queries~\citep{HardtT}, robust regression~\citep{AsiD}, some combinatorial optimization problems~\citep{GuptaLMRT}, $k$-means clustering~\citep{FeldmanFKN}, optimization of dispersed functions~\citep{BalcanDV}, convex optimization~\citep{BassilyST, MinamiASN16}, Bayesian data analysis~\citep{Mir, DimitrakakisNMR, WangFS15, WassermanZ, FouldsGWC}, linear and quantile regression~\citep{ReimherrA}, etc.

Implementing these mechanisms requires sampling from a distribution given by $\exp(-f)$ from some domain $D$, for a suitable score function $f$. When the domain $D$ is finite and small, this sampling is straightforward. Several differentially private mechanisms instantiate the exponential mechanism where $D=\mathbb{R}^d$, in which case this sampling is not straightforward.

Such sampling problems are not new and often occur in statistics and machine learning settings. The common practical approach is to use heuristic MCMC samplers such as Gibbs sampling, which often works well in problems arising in practice. However, given that convergence is not guaranteed, the resulting algorithms may not be differentially private. Indeed one can construct simple score functions on the hypercube for which the natural Metropolis chain run for any polynomial time leads to a non-private algorithm~\citep{GaneshT}. There are also well-known complexity-theoretic barriers in exactly sampling from $\exp(-f)$ if $f$ is not required to be convex. 

Several applications however involve convex functions $f$ and this is the focus of the current work. Indeed this is the problem of sampling from a log-concave distribution, which has attracted a lot of interest. Here, there are two broad lines of work. The classical results in this line of work (e.g. ~\citep{ApplegateK91, LovaszV07}) show that given an oracle for computing the function, one can sample from a distribution that is $\eps$-close\footnote{The letter $\eps$ commonly denotes the privacy parameter in DP literature, and the  distance to the target distribution in the sampling literature. Since most of the technical part of this work deals with sampling, we will reserve $\eps$ for distance, and will let $\privacyparam$ denote the privacy parameter.} 
to the target distribution in time polynomial in $d$ and $\log \frac 1 \eps$. Here the closeness is measured in statistical distance. By itself, this does not suffice to give a differentially private algorithm, as DP requires closeness in more stringent notions of distance. The fact that run time is logarithmic in $\frac 1 \eps$ however allows for an exponentially small statistical distance in polynomial time. This immediately yields $(\privacyparam, \delta)$-DP algorithms, and with some additional work can also yield $\privacyparam$-DP algorithms~\citep{HardtT}. Techniques from this line of work can also sometimes apply to non-convex $f$ of interest. Indeed~\citet{KapralovT} designed a polynomial time algorithm for the case of $f$ being a Rayleigh quotient to allow for efficient private PCA.

The runtime of these log-concave sampling algorithms however involves large polynomials. A beautiful line of work has reduced the dependence (of the number of function oracle calls) on the dimension from roughly $d^{10}$ in~\citet{ApplegateK91} to $d^3$ in~\citet{LovaszV06, LovaszV07}. Nevertheless, the algorithms still fall short of being efficient enough to be implementable in practice for large $d$. A second, more recent, line of work ~\citep{Dalalyan16,DurmusM19} have shown that ``first order'' Markov Chain Monte Carlo (MCMC) algorithms such as Langevin MCMC and Hamiltonian MCMC enjoy fast convergence, and have better dependence on the dimension. These algorithms are typically simpler and more practical but have polynomial dependence on the closeness parameter $\eps$. This polynomial dependence on $\eps$ makes the choice of distance more important. Indeed these algorithms have been analyzed for various measures of distance between distributions such as statistical distance, KL-divergence and Wasserstein distance.

These notions of distance however do not lead to efficient differentially private algorithms (see~\cref{app:distance_measures} in supplementary materials). This motivates the question of establishing rapid mixing in \Renyi divergence for these algorithms. This is the question we address in this work, and show that when $f$ is smooth and strongly convex, discretized Langevin dynamics converge in iteration complexity near-linear in the dimension. This gives more efficient differentially private algorithms for sampling for such $f$.

\citet{VempalaW19} recently studied this question for similar reasons. They considered the Unadjusted (i.e., overdamped) Langevin Algorithm and showed that when the (discretized) Markov chain satisfies suitable mixing properties (e.g. Log Sobolev inequality), then the discrete process converges in \Renyi divergence to {\em a} stationary distribution. However this stationary distribution of the discretized chain is different from the target distribution. The \Renyi divergence between the stationary distribution and $\exp(-f)$ is not very well-understood~\citep{RobertsT1996, Wibisono18}, and it is conceivable that the stationary distribution of the discrete process is {\em not} close in \Renyi divergence to the target distribution and thus may not be differentially private. Thus the question of designing fast algorithms that sample from a distribution close to the distribution $\exp(-f)$ in \Renyi divergence was left open.

In this work we use a novel approach to address these questions of fast sampling from $\exp(-f)$ using the discretized Langevin Algorithm. Interestingly, we borrow tools commonly used in differential privacy, though applied in a way that is not very intuitive from a privacy point of view. We upper bound the \Renyi divergence between the output of the discrete Langevin Algorithm run for $T$ steps, and the output of the continuous process run for time $T \eta$. The continuous process is known~\citep{VempalaW19} to converge very quickly in \Renyi divergence to the target distribution. This allows us to assert closeness (in \Renyi divergence) of the output of the discrete algorithm to the target distribution.  This bypasses the question of the bias of the stationary distribution of the discrete process. Moreover, this gives us a differentially private algorithm with iteration complexity near-linear in the dimension. Our result applies to log-smooth and strongly log-concave distributions. While results of this form may also be provable using methods from optimal transport, we believe that our techniques are simpler and more approachable to the differential privacy community, and may be more easily adaptable to other functions $f$ of interest.

Our approach is general and simple. We show that it can be extended to the {\em underdamped} Langevin dynamics which have a better dependence on dimension, modulo proving fast mixing for the continuous process. As specific applications, we show how our results lead to faster algorithms for the implementing the mechanisms in~\citet{MinamiASN16}.



%[Re. stationary distribution, or more generally for larger $T$: can we not argue that (A) the distribution after $\tau$ steps is close in Renyi for a suitable $\tau$. (B) if we start for this distribution, this is a good warm start so doing our analysis for the next $\tau$ steps, we maintain this property. Also, this inductively should imply that the stationary distribution has good renyi.]\arun{We use triangle inequality to show that if our starting $2\alpha$-divergence is small, the final $\alpha$-divergence of the discrete chain is small, so induction gets pretty bad}

As is common in this line of work, we ignore numerical issues and assume real arithmetic. The results can be translated to the finite-precision arithmetic case by standard techniques, as long as the precision is at least logarithmic in $d$ and $T$. The real arithmetic assumption thus simplifies the presentation without affecting the generality of the results.

\subsection*{Other Related Work} %% Not sure if we want to put too much else here so making it a sentence.
%
\citet{WangFS15} discuss the issue of privacy when using approximate samplers at length and consider two algorithms. The first one (OPS) that samples approximately from $\exp(-f)$ considers closeness in statistical distance and thus can only be efficient when coupled with the first kind of samplers above, i.e. those that have a logarithmic dependence on the closeness parameter. The second algorithm they analyze is a variant of Stochastic Gradient Langevin Dynamics (SGLD). The algorithm adds additional noise for privacy, and while it is shown to be private for suitable parameters, it does not ensure convergence to the target distribution. Differentially private approximations to SGLD have also been studied in~\cite{LiCLC}. Note that in contrast, we do not need to modify the Langevin dynamics which ensures convergence as well as privacy.

There is a large body of work on Langevin algorithms and their variants. We refer the reader to the surveys by~\citet{roberts2004} and~\citet{Vempala05geometricrandom}. There has been a recent spate of activity on analyzing these algorithms and their stochastic variants, under different kinds of assumptions on $f$ and we do not attempt to summarize it here.


% ------------------Old intro-------

% In this work, we study the problem of sampling from a logconcave distribution. This is an important and well-studied problem and there are polynomial time algorithms for the problem~\citep{ApplegateK91, LovaszV07}. In recent years, the problem has attracted renewed interest and a sequence of works~\citep{Dalalyan16,DurmusM19} have shown that ``first order'' Markov Chain Monte Carlo (MCMC) algorithms such as Langevin MCMC and Hamiltonian MCMC enjoy fast convergence, and have better dependence on the dimension.

% One motivation for sampling from such distributions comes from the application of these sampling procedures to the design of Differentially Private Algorithms. The Exponential mechanism~\citep{McSherryT07} is a general algorithm in differential privacy that requires sampling from the distribution proportional to $\exp(-f(\bx))$ for an appropriate $f$. When $f$ is convex, as is the case in some applications of the exponential mechanism and its variants ~\citep{WangFS15,MinamiASN16}, this problem translates to sampling from a log concave distribution.

% Existing algorithms for sampling from logconcave distributions are known to output samples from a distribution that is close to the intended distribution. The closeness is typically measured in statistical distance, Wasserstein distance, or in KL divergence. Unfortunately, none of these distances are strong enough to ensure differential privacy for the resulting algorithm. The more stringent choice of distance in differential privacy is for a good reason: it is easy to construct examples of algorithms that ensure privacy with respect to one of these weaker notions of distance but are clearly unsatisfactory from a privacy point of view~\citep{DworkRbook}. This motivates the question of efficient sampling in terms of a stronger measure of distance such as $\infty$-divergence, or \Renyi divergence (both of which upper bound KL divergence and thus upper bound statistical distance and Wasserstein distances). Different distance notions can be related to each other and~\citet{HardtT} showed that an exponentially small statistical distance guarantee suffices to derive a differentially private algorithm. Given that there are sampling algorithms that have a $\log \delta^{-1}$ type dependence on the statistical distance $\delta$, this can be used to derive polynomial time differentially private versions of the exponential mechanism in these settings. However, the polynomials are high-degree resulting in an impractical algorithm.

% This led~\citet{VempalaW19} to study the convergence in \Renyi divergence for the faster Langevin dynamics algorithm. They considered the Unadjusted Langevin Algorithm and showed that when the (discretized) Markov chain satisfies suitable mixing properties (e.g. Log Sobolev inequality), then the discrete process converges in \Renyi divergence to its stationary distribution. However the stationary distribution of the discretized chain is different from the target distribution and this issue of {\em bias} makes it difficult to argue the required mixing properties. Further the \Renyi divergence resulting from this bias is poorly understood~\citep{RobertsT1996, Wibisono18}, and it is conceivable that the stationary distribution of the discrete process is {\em not} close in \Renyi divergence to the target distribution. In fact, we do not even know if the stationary distribution of the discrete process is differentially private. Thus the question of designing fast algorithms that sample from a distribution close to the distribution $\exp(f)$ in \Renyi divergence is open.

% In this work we use a novel approach to address these questions of fast sampling and understanding the bias of the discretized Langevin Algorithm. Interestingly, we borrow tools commonly used in differential privacy, though applied in a way that is not very intuitive from a privacy point of view. We upper bound the \Renyi divergence between the output of the discrete Langevin Algorithm run for $t$ steps, and the output of the continuous process run for time $\eta t$. The continuous process is known~\citep{VempalaW19} to converge very quickly in \Renyi divergence to the target distribution. This allows us to assert closeness (in \Renyi divergence) of the output of the discrete algorithm to the target distribution.  This bypasses the question of the bias of the stationary distribution of the discrete process. Moreover, this gives us a differentially private algorithm with iteration complexity linear in the dimension. Our result applies to log smooth and strongly log concave distributions.

% Our approach is general and simple. We show that it can be extended to the {\em underdamped} Langevin dynamics which have a better dependence on dimension, modulo proving fast mixing for the continuous process.

% Our work raises several interesting questions. While our bounds are for log smooth and strongly log concave distributions, it would be interesting to relax these assumptions. The known results for the continuous process in the underdamped case are only for weaker measures, and it is compelling to extend them to \Renyi divergence. Our result has a seemingly curious property: the finite time behaviour of the discrete chain is shown to be close in \Renyi divergence to the target distribution, yet we do not know if the stationary distribution of the discrete chain satisfies this property. This is reminiscent of some results in privacy literature, where e.g., running noisy SGD for a fixed number of steps can be shown to be private but we know nothing of the privacy if we run noisy SGD for many more steps~\citep{BassilyST,FeldmanMTT18}. Addressing this gap in our understanding is left to future work. Finally, there are several variants of these methods that have been studied (e.g. Metropolis Adjusted Langevin Algorithm, Hamiltonian Monte Carlo) and extending our techniques to these methods would be interesting.

% As is common in this line of work, we ignore numerical issues and assume real arithmetic. The results can be translated to the finite-precision arithmetic case by standard techniques, as long as the precision is at least logarithmic in $d$ and $T$. The real arithmetic assumption thus simplifies the presentation without affecting the generality of the results.

% %\subsection{Other Related Work}. %% Not sure if we want to put too much else here so making it a sentence.
% There is a large body of work on Langevin algorithms and their variants. We refer the reader to the surveys by~\citet{roberts2004} and~\citet{Vempala05geometricrandom}. There has been a recent spate of activity on analyzing these algorithms and their stochastic variants, under different kinds of assumptions on $f$ and we do not attempt to summarize it here.


% Sampling from distributions ke $\exp(-f)$ is important.
% Lots of recent interest in Langevin dynamics methods.
% Bias issue. tricky.

% For many applications, including for DP applications, want convergence in a strong sense. SD or even KL not sufficient. Would like Renyi convergence.

% Existing approaches based on sampling from log concave distribution are not super efficient and translating the SD bounds they get to measures more appropriate for privacy loses large polynomial factors.

% This question has previously been addressed by VW. They show ...

%In this work we present a different approach to this question. We show that the discrete process closely tracks the continuous one by using tools from privacy. combined with fast mixing of the continuous process, this allows us to prove strong upper bounds. Our bounds are similar to those proved for weaker notions of distance such as KL or SD. 

%Our approach is general and simple, and complementary to the VW approach. At heart their approach shows that at each step the discrete process gets closer to its stationary distribution up to some small error. This leaves the question of the stationary process's stationary distribution itself. Additionally, this mixing time type analysis can only work for large enough $T$ so that the discrete process mixes; this in turn requires VW to assume specific properties of the discrete process that would allow them to prove fast mixing (LSI or Poincare).
%Our approach is fundamentally different and tracks the divergence between the discrete and the continuous processes. These bounds slowly degrade with the number of steps, and hold for small enough $T$. Since the continuous process can be shown to mix quickly in Renyi, this allows us to prove fast convergence bounds. Our result applies to smooth and strongly convex functions $f$.

%Results

%Techniques

%Open questions.

%Related work in other measures

%This kind of arguments which degrade with $T$ are common in DP (examples).


\subsection*{Results and Techniques}
%
\begin{figure}
\begin{center}
\begin{tabular}{|l|l|c|c|}
\hline
$f$ is $L$-smooth and & Process & $\eta$ & Iterations\\
\hline
1-strongly convex & Overdamped  & $\tilde{O}\left(\frac{1}{\tau L^4 \ln^2 \alpha} \cdot \frac{\eps^2}{d} \right)$ (Thm~\ref{lemma:conditionaldivergence}) & $\tilde{O}\left(\frac{d \tau^2 L^4 \ln^2 \alpha}{\eps^2} \right)$ \\
\hline
$B$-Lipschitz     & Overdamped  & $\tilde{O}\left(\frac{1}{\tau L^4 \ln^2 \alpha} \cdot \frac{\eps^2}{B^2 + d} \right)$ (Thm~\ref{lemma:conditionaldivergence-lipschitz})& $\tilde{O}\left(\frac{(B^2 + d) \tau^2 L^4 \ln^2 \alpha}{\eps^2} \right)$ \\
\hline
1-strongly convex & Underdamped &  $\tilde{O}\left(\frac{1}{\tau L \ln \alpha} \cdot \frac{\eps}{\sqrt{d}} \right)$ (Thm~\ref{lemma:conditionaldivergence-ud}) & $\tilde{O}\left(\frac{\sqrt{d} \tau^2 L \ln \alpha}{\eps} \right)$ \\
\hline
\end{tabular}
\end{center}
\caption{Summary of results. For each family of functions and process (either overdamped or underdamped Langevin dynamics), an upper bound is listed on the step size $\eta$ (and thus a bound on the iteration complexity) needed to ensure the $\alpha$-R\'enyi divergence between the discrete and continuous processes is at most $\eps$ after time $\tau$. Setting $\alpha = O(\ln(1/\delta)/\privacyparam), \eps = \privacyparam/2$ gives that the $\delta$-approximate max divergence is at most $\privacyparam$, i.e. $(\privacyparam, \delta)$-differential privacy.\vspace{-0.2in}}
\label{fig:results}
\end{figure}

Our results are summarized in Figure~\ref{fig:results}. Combined with results from \cite{VempalaW19} on the convergence of the continuous process, the first result gives the following algorithmic guarantee, our main result:

\begin{theorem}\label{thm:mainthm}
Fix any $\alpha \geq 1$. Let $R$ be a distribution satisfying $R(x) \propto e^{-f(x)}$ for 1-strongly convex and $L$-smooth $f$ with global minimum at 0. Let $P$ be the distribution arrived at by running discretized overdamped Langevin dynamics using $f$ with step size $\eta = \tilde{O}(\frac{1}{\tau L^4 \ln^2 \alpha} \cdot \frac{\eps^2}{d})$ for continuous time $\tau = \alpha \ln \frac{d \log L}{\eps}$ (i.e. for $\tilde{O}(\frac{\alpha^2 L^4 d}{\eps^2})$ steps) from initial distribution $N(0, \frac{1}{L}I_d)$. Then we have $D_\alpha(P || R) \leq \eps$.
\end{theorem}

This is the first algorithmic result for sampling from log-smooth and strongly log-concave distributions with low error in R\'enyi divergence without additional assumptions. All results in Figure~\ref{fig:results} are achieved using a similar analysis, which we describe here.
Instead of directly bounding the divergence between the discrete and continuous processes, we instead bound the divergence between the discrete processes using step sizes $\eta, \eta/k$. Our resulting bound does not depend on $k$, so we can take the limit as $k$ goes to infinity and the latter approaches the continuous process. Suppose within each step of size $\eta$, neither process moves more than $r$ away from the position at the start of this step. Then by smoothness, in each interval of length $\eta/k$ the distance between the gradient steps between the two processes is upper bounded by $Lr \frac{\eta}{k}$. Our divergence bound thus worsens by at most $D_\alpha(N(0, \frac{2\eta}{k}) ||  N(x, \frac{2\eta}{k}))$ where $x$ is a vector with $\norm{x}_2 \leq Lr \frac{\eta}{k}$. The divergence between shifted Gaussians is well-known, giving us a divergence bound. 

Of course, since the movement due to Brownian motion can be arbitrarily large, there is no unconditional bound on $r$. Instead, we derive tail bounds for $r$, giving a divergence bound (depending on $\delta$) between the two processes conditioned on a probability $1 - \delta$ event for every $\delta$. We then show a simple lemma which says that conditional upper bounds on the larger moments of a random variable give an unconditional upper bound on the expectation of that random variable. By the definition of R\'enyi divergence, $\exp((\alpha' - 1) D_{\alpha'}(P || Q))$ is a moment of $\exp((\alpha - 1) D_{\alpha}(P || Q))$ for $\alpha' > \alpha$, so we can apply this lemma to our conditional bound on $\alpha'$-R\'enyi divergence to get an unconditional bound on $\alpha$-R\'enyi divergence via Jensen's inequality. 

Finally, since our analysis only needs smoothness, the radius tail bound, and the fact that the process is a composition of gradient steps with Gaussian noise, our analysis easily extends to sampling from Lipschitz rather than strongly convex functions and analyzing the underdamped Langevin dynamics.

As an immediate application, we recall the work of~\citet{MinamiASN16}, who give a differentially private mechanism that (approximately) samples from Gibbs posterior with a strongly log-concave prior, for applications such as mean estimation and logistic regression. Their iteration complexity of $\tilde{O}(d^3/\delta^2)$ proved in~\citet[Prop. 13]{MinamiASN16} gets improved to $\tilde{O}(d/\privacyparam^4)$ using our main result. We note that the privacy parameters in $(\privacyparam, \delta)$-DP that one typically aims for are $\privacyparam$ being constant, and $\delta$ being negligible.

We start with some preliminaries in~\cref{section:prelim}. We prove a ``one-sided'' version of the main result in~\cref{section:bounded} and~\cref{section:odconvergence}, and prove the result for the underdamped case in~\cref{sec:underdamped}. We discuss future research directions in~\cref{section:discussion}. We defer proofs and some additional preliminaries to the supplementary material.
% We consider the problem of (approximately) sampling from the distribution on $\mathbb{R}^d$ with density function $p$ satisfying $p(x) \propto e^{-f(x)}$. It is well known that the continuous random process given by the stochastic differential equation

% $$ \D{x_t} = -\grad f(x_t) \D{t} + \sqrt{2} \D{B_t},$$

% known as the overdamped Langdevin dynamics, has stationary distribution $p$ under mild assumptions (here $B_t$ is the standard Brownian motion in $\mathbb{R}^d$). We analyze the convergence of the (efficiently implementable) discretized version of overdamped Langevin dynamics with step size $\eta$, given by

% $$ \D{x_t} = -\grad f(x_{\lfloor \frac{t}{\eta}\rfloor \eta}) \D{t} + \sqrt{2} \D{B_t}.$$

% Equivalently, if we only care about times at multiples of $\eta$ $x_i' = x_{i\eta}$:

% $$x_{i+1}' \sim N(x_i' - \eta \grad f(x_i'), 2\eta I_d).$$

% Our analysis is for $f$ that is twice-differentiable, $m$-strongly convex, and $L$-smooth (i.e. $mI_d \psdleq \grad^2 f \psdleq LI_d$). Without loss of generality, we will assume that the global minimum of $f$ is $f(\bzero) = 0$: If $x^*$ is the true global minimum, we can efficiently find $x^*$ using e.g. gradient descent. Then, we can sample from the function with density proportional to $e^{-g(x)}$ for $g(x) := f(x - x^*) - f(x^*)$, which does have global minimum $g(\bzero) = 0$, and shift our sample by $x^*$ to get a sample from $p$. We will also assume without loss of generality that $m = 1$, since the function $g(x) := f(\frac{1}{m}x)$ is 1-strongly convex and $L/m$-smooth, and we can sample $x$ from the function with density proportional to $e^{-g(x)}$ and rescale by $m$ to get a sample from $p$. Convergence bounds for sampling from $m$-strongly convex and $L$-smooth functions are often given as functions of the condition number $L/m$ - by this assumption, we can instead represent the condition number by just $L$.

==> prelim.tex <==
\section{Preliminaries}

\subsection{Langevin Dynamics and Basic Assumptions}

For the majority of the paper we focus on the overdamped Langevin dynamics, given by the following stochastic differential equation (SDE):

$$ \D{x_t} = -\grad f(x_t) \D{t} + \sqrt{2} \D{B_t},$$

Where $B_t$ is a standard $d$-dimensional Brownian motion. Under mild assumptions, it is known that the stationary distribution of the SDE is the distribution $p$ satisfying $p(x) \propto e^{-f(x)}$. Algorithmically, it is easier to use the following discretization with \textit{timesteps} of length $\eta$:

$$ \D{x_t} = -\grad f(x_{\lfloor \frac{t}{\eta}\rfloor \eta}) \D{t} + \sqrt{2} \D{B_t},$$

i.e., we only update the position whose gradient is used in the SDE at the beginning of each timestep. Restricted to the position at times that are multiples of $\eta$, equivalently:

$$x_{(i+1)\eta} = x_{i \eta} - \eta \grad f(x_{i \eta}) + \xi_i.$$

Where $\xi_i \sim N(0, 2\eta I)$ are independent samples. Throughout the paper, when we refer to the result of running a Langevin dynamics for \textit{continuous time $t$}, we mean the distribution $x_t$, \textit{not} the distribution $x_{t \eta}$. When the iteration complexity (i.e. number of timesteps) is of interest, we may refer to running a Langevin dynamics for continuous time $T\eta$ equivalently as the result of running it for $T$ timesteps.

A similarly defined second order process is the underdamped Langevin dynamics, given by the following SDE (parameterized by $\gamma, \mu > 0$):

$$\D v_t = -\gamma v_t \D t - \mu \grad f(x_t) \D t + \sqrt{2 \gamma \mu} \D B_t, \qquad \D x_t = v_t \D t.$$

Algorithmically, it is easier to use the following discretization:

$$\D v_t = -\gamma v_t \D_t - \mu \grad f(x_{\lfloor \frac{t}{\eta} \rfloor \eta}) \D t + \sqrt{2 \gamma \mu} \D B_t, \qquad \D x_t = v_t \D t.$$

In the majority of the paper we consider sampling from distributions given by $m$-strongly convex, $L$-smooth functions $f$. To simplify the presentation, we also assume $f$ is twice-differentiable, so these conditions on $f$ can be expressed as: for all $x$, $mI \psdleq \grad^2 f(x) \psdleq LI$. We make two additional simplifying assumptions: The first is that the stationary point of $f$ is at $0$, as if $f$'s true stationary point is $x^* \neq 0$, we can sample from $g(x) := f(x - x^*)$ and then shift our sample by $x^*$ to get a sample from $f$ instead ($x^*$ or a low-error estimate which suffices can be found using e.g. gradient descent). The second is that $m = 1$, as if $m \neq 1$, we can sample from $g(x) = f(\frac{1}{\sqrt{m}}x)$ and rescale our sample by $\sqrt{m}$ instead.

\subsection{R\'enyi Divergence}

\begin{definition}[R\'enyi Divergence]
For $0 < \alpha < \infty$, $\alpha \neq 1$ and distributions $\mu, \nu$, such that $\supp(\mu) = \supp(\nu)$ the $\alpha$-R\'enyi divergence between $\mu$ and $\nu$ is

$$ D_\alpha(\mu || \nu) = \frac{1}{\alpha - 1} \ln \int_{\supp(\nu)} \frac{\mu(x)^\alpha}{\nu(x)^{\alpha - 1}} \D{x} = \frac{1}{\alpha - 1} \ln \ex_{x \sim \nu}\left[ \frac{\mu(x)^\alpha}{\nu(x)^\alpha}\right].$$

The $\alpha$-R\'enyi divergence for $\alpha = 1$ (resp. $\infty$) is defined by taking the limit of $D_\alpha(\mu||\nu)$ as $\alpha$ approaches $1$ (resp. $\infty$) and equals the KL divergence (resp. max divergence).
\end{definition}

R\'enyi divergence is a standard notion of divergence in information theory, and bounds on R\'enyi divergence translate immediately to $(\epsilon,\delta)$-differential privacy bounds. We recall some standard facts about R\'enyi divergences.

\begin{fact}[Monotonicity {\cite[Theorem 3]{vanErvenH14}}]
For any distributions $P, Q$ and $0 \leq \alpha_1 \leq \alpha_2$ we have $D_{\alpha_1}(P || Q)$ $\leq D_{\alpha_2}(P||Q)$. 
\end{fact}

\begin{fact}[Post-Processing {\cite[Theorem 9]{vanErvenH14}}]\label{fact:postprocessing}
For any sample spaces $\mathcal{X}, \mathcal{Y}$, distributions $X_1, X_2$ over $\mathcal{X}$, and any function $f:\mathcal{X} \rightarrow \mathcal{Y}$ we have $D_\alpha(f(X_1) ||f(X_2)) \leq D_\alpha(X_1 || X_2)$.
\end{fact}

\begin{fact}[Gaussian Divergence {\cite[Example 3]{vanErvenH14}}]\label{fact:gaussiandivergence}
Recall that the $\infty$-Wasserstein distance between two distributions $p, q$ (using a given norm on the support of $p, q$) is defined as 

$$W_\infty(p, q) = \inf_{\gamma \in \Gamma(p, q)} \sup_{(x, y) \in \supp(\gamma)} \norm{x - y},$$ 

Where $\Gamma(p, q)$ denotes the set of couplings of $p$ and $q$. Let $p, q$ be any distributions over $\mathbb{R}^d$ with $\infty$-Wasserstein distance $W_\infty(p , q) \leq r$ (using the $\ell_2$-norm). Then $D_\alpha(p \ast N(0, \sigma^2 I_d) || q \ast N(0, \sigma^2 I_d)) \leq \frac{\alpha r^2}{2\sigma^2}$. 
\end{fact}

\begin{fact}[Adaptive Composition Theorem {\cite[Proposition 1]{Mironov2017}}]\label{fact:composition}
Let $\mathcal{X}_0,$ $\mathcal{X}_1, \ldots, \mathcal{X}_k$ be arbitrary sample spaces. For each $i \in [k]$, let $f_i, f_i':\Delta(\mathcal{X}_{i-1}) \rightarrow \Delta(\mathcal{X}_i)$ be maps from distributions over $\mathcal{X}_{i-1}$ to distributions over $\mathcal{X}_i$ such that for any distribution $X_{i-1}$ over $\mathcal{X}_{i-1}$, $D_\alpha(f_i(X_{i-1}) || f_i'(X_{i-1})) \leq \epsilon_i$. Then, for $F, F':\Delta(\mathcal{X}_0) \rightarrow \Delta(\mathcal{X}_k)$ defined as $F(\cdot) = f_k(f_{k-1}( \ldots f_1(\cdot) \ldots )$ and $F'(\cdot) = f'_k(f'_{k-1}( \ldots f'_1(\cdot) \ldots )$ we have $D_\alpha(F(X_0) || F'(X_0)) \leq \sum_{i=1}^k \epsilon_i$ for any $X_0 \in \Delta(\mathcal{X}_0)$.
\end{fact}

\begin{fact}[Weak Triangle Inequality {\cite[Proposition 11]{Mironov2017}}]
For any $\alpha > 1$, $p, q > 1$ satisfying $1/p + 1/q = 1$ and distributions $P, Q, R$ with the same support:

$$D_\alpha(P||R) \leq \frac{\alpha - 1/p}{\alpha - 1}D_{p\alpha}(P||Q) + D_{q(\alpha - 1/p)}(Q||R).$$
\end{fact}

\begin{definition}[Approximate Differential Privacy]\label{definition:apxdp}
Let $X$ be any set. $N:X \rightarrow 2^X$ be a perturbation set, and $\mathcal{Y}$ be a sample space. Then a mechanism $\mathcal{M}:X \rightarrow \Delta(\mathcal{Y})$ is $(\epsilon, \delta)$-differentially private if for any $x \in X, x' \in N(x)$, $S \subseteq \mathcal{Y}$:

$$\Pr_{y \sim \mathcal{M}(x)}[y \in S] \leq e^\epsilon \cdot \Pr_{y \sim \mathcal{M}(x')}[y \in S] + \delta.$$
\end{definition}

\begin{fact}[{\cite[Proposition 3]{Mironov2017}}]
Let $X, N, \mathcal{Y}$ be defined as in Definition~\ref{definition:apxdp}. If $\mathcal{M}$ satisfies that for any $x, x' \in N(x)$:

$$D_\alpha(\mathcal{M}(x) || \mathcal{M}(x')) \leq \epsilon,$$

Then $\mathcal{M}$ is $(\epsilon + \frac{\log 1/\delta}{\alpha - 1}, \delta)$-differentially private for $0 < \delta < 1$.
\end{fact}

Some proofs in the appendix use additional well-known facts. These facts are deferred to Appendix~\ref{section:prelim-def}.

%The following observation will be useful in relating the divergence between $\mu, \nu$ and the divergence between $\mu, \nu$ conditioned on some high-probability event:

% \begin{observation}
% If $\supp(\mu) = \supp(\nu)$, then:

% $$\int_{\supp(\nu)}\frac{\mu(x)^\alpha}{\nu(x)^{\alpha - 1}} \ \D{x} = \ex_{x \sim \mu} \ex_{y \sim \text{Unif}(0, \mu(x))} \left[\frac{\alpha y^{\alpha - 1}}{\nu(x)^{\alpha - 1}}\right].$$

% \end{observation}
% \begin{proof}
% $$\ex_{x \sim \mu} \ex_{y \sim \text{Unif}(0, \mu(x))} \left[\frac{\alpha y^{\alpha - 1}}{\nu(x)^{\alpha - 1}}\right] = \int_{\supp(\mu) } \mu(x) \ex_{y \sim \text{Unif}(0, \mu(x))} \left[\frac{\alpha y^{\alpha - 1}}{\nu(x)^{\alpha - 1}}\right] \D{x} =$$
% $$\int_{\supp(\mu)} \mu(x) \int_0^{\mu(x)} \frac{1}{\mu(x)}\frac{\alpha y^{\alpha - 1}}{\nu(x)^{\alpha - 1}} \D{y}\ \D{x}= \int_{\supp(\mu)}\frac{1}{\nu(x)^{\alpha - 1}} \int_0^{\mu(x)} \alpha y^{\alpha - 1} \D{y}\ \D{x}=  $$
% $$\int_{\supp(\mu)}\frac{\mu(x)^\alpha}{\nu(x)^{\alpha - 1}} \ \D{x} = \int_{\supp(\nu)}\frac{\mu(x)^\alpha}{\nu(x)^{\alpha - 1}} \ \D{x}.$$
% \end{proof}

% Note that $(x, y)$ is distributed uniformly over all pairs $x, y$ such that $0 \leq y \leq \mu(x)$.

% To avoid introducing new terminology, we ignore the requirement that norms are scalable:

% \begin{definition}
% A function $\norm{\cdot}: \mathbb{R}^d \rightarrow \mathbb{R}_{\geq 0}$ is (abusing terminology) a norm if it satisfies positive definiteness and triangle inequality \textit{but not necessarily scalability}, i.e. $\norm{x} = 0$ if and only if $x = \bzero$ and $\norm{x + y} \leq \norm{x} + \norm{y}$, but $\norm{cx}$ is not necessarily equal to $|c| \cdot \norm{x}$ for all $x$.
% \end{definition}

% For our purposes the Wasserstein distance between two measures with respect to a norm is well-defined independent of the scalability property of norms, so we can reproduce the following definition from \cite{FeldmanMTT18}:

% \begin{definition}[Shifted R\'enyi Divergence]
% For distributions $\mu, \nu$ with support on $\mathbb{R}^d$ endowed with norm $\norm{\cdot}$, the $z$-shifted $\alpha$-R\'enyi divergence between $\mu$, $\nu$ is

% $$D_\alpha^{(z)}(\mu || \nu) = \inf_{\mu': W_{\infty}(\mu, \mu') \leq z} D_{\alpha}(\mu' || \nu).$$

% \end{definition}

% \begin{definition}
% For distribution $\zeta$ defined on $\mathbb{R}^d$ endowed with norm $\norm{\cdot}$, we denote the largest $\alpha$-R\'enyi divergence between $\zeta$ and $\zeta$ shifted by a vector of norm at most $a$ by

% $$R_\alpha(\zeta, a) := \sup_{x: \norm{x} \leq a} D_\alpha(\zeta \ast x || \zeta).$$

% \end{definition}

% \subsection{Contractive Noisy Iteration}

% We analyze the discretized version of Langevin dynamics by viewing it as a type of Contractive Noisy Iteration (Definition 19 in \cite{FeldmanMTT18}). We write the definition here for a random variable in $\mathbb{R}^d$. 

% \begin{definition}[Contractive Noisy Iteration]\label{def:cni}
% Given an initial random state $X_0 \in \mathbb{R}^d$, a sequence of contractive functions $\psi_t: \mathbb{R}^d \rightarrow \mathbb{R}^d$, a sequence of noise distributions $\{\zeta_t\}$, and a sequence of maps $f_t: \mathbb{R}^d \rightarrow \mathbb{R}^d$ Contractive Noisy Iteration is the random variable sequence given by the following rule:

% $$X_{t} = \Psi_t(\psi_t(X_{t-1}) + Z_{t}), Z_{t} \sim \zeta_{t}.$$

% We refer to the distribution of $X_T$ as $CNI_T(X_0, \{\psi_t\}, \{\zeta_t\}, \{\Psi_t\})$.
% \end{definition}

% Our definition adds the generalization that additional maps $\Psi$ can be applied in the middle of the process. We will eventually compare CNI instances with the same $\zeta, \Psi$ but differing $\psi$. Because they are deterministic and do not differ between the two instances, by the post-processing property of R\'enyi-divergence applying them can only reduce the divergence between distributions, hence there is no need for them to be contractive like the maps $\psi$. In particular, we cget the following as a corollary of \cite{FeldmanMTT18}. 

% \begin{theorem}\label{thm:cnidivergence}
% Let $X_T$ and $X_T'$ denote the random variables $CNI_T(X_0, \{ \psi_t\}, \{\zeta_t\}, \{\Psi_t\})$ and $CNI_T(X_0,$ $\{ \psi'_t\}, \{\zeta_t\}, \{\Psi_t\})$ defined over $\mathbb{R}^d$ endowed with norm $\norm{\cdot}$. Suppose that $\psi_t, \psi_t'$ that are contractive. Let $s_t = \sup_{x \in \supp(X_{t-1})} \norm{\psi_t(x) - \psi_t'(x)}$. Then:

% $$D_\alpha(X_T || X'_T) \leq \sum_{t = 1}^T R_\alpha (\zeta_t, s_t).$$

% \end{theorem}
% \begin{proof}
% There are three modifications from the result in \cite{FeldmanMTT18}: 
% \begin{itemize}
%     \item The addition of the deterministic maps $\Psi_t$ to the CNI process.
%     \item The removal of the scalability requirements for norms.
%     \item Only requiring that $\norm{\psi_t(x) - \psi_t'(x)}$ is bounded in $\supp(X_{t-1})$ rather than all of $\mathbb{R}^d$.
% \end{itemize}

% The first modification is fine because of the post-processing property of R\'enyi divergence. The second modification is fine because the proofs in \cite{FeldmanMTT18} of Theorem~\ref{thm:cnidivergence} never use the scalability property. The third modification is fine because the only application of the requirement that $\norm{\psi_t(x) - \psi_t'(x)}$ is bounded by $s_t$ in all of $\mathbb{R}^d$ is used to show that:

% $$D_\alpha^{(z+s_t)}(\psi_t (X_{t-1}) || \psi'_t (X_{t-1}')) \leq D_\alpha^{(z)}(X_{t-1} || X_{t-1}')$$

% This can still be shown with the relaxed requirement that $\norm{\psi_t(x) - \psi_t'(x)}$ is bounded in $\supp(X_{t-1})$ by modifying the original proof slightly: There exists $Y$ such that $\norm{X_{t-1} - Y} \leq z$ with probability 1, and $D_\alpha(Y, X_{t-1}) = D_\alpha^{(z)}(X_{t-1} || X_{t-1}')$. By post-processing, $D_\alpha^{(z)}(\psi'_t(Y) || \psi'_t(X_{t-1}')) \leq D_\alpha(Y, X_{t-1})$. It suffices to show $W_\infty (\psi_t(X_{t-1}), \psi'_t(Y)) \leq z+s_t$. This follows because:

% $$\norm{\psi_t(X_{t-1}) - \psi_t'(Y)} \leq \norm{\psi_t(X_{t-1}) - \psi'_t(X_{t-1})} + \norm{\psi'_t(X_{t-1}) - \psi'_t(Y)} \leq s_t + \norm{X_{t-1} - Y} \leq s_t + z.$$

% \end{proof}
